Online Conversion with Switching Costs: Robust and Learning-Augmented Algorithms

We introduce and study online conversion with switching costs, a family of online problems that capture emerging problems at the intersection of energy and sustainability. In this problem, an online player attempts to purchase (alternatively, sell) fractional shares of an asset during a fixed time horizon with length $T$. At each time step, a cost function (alternatively, price function) is revealed, and the player must irrevocably decide an amount of asset to convert. The player also incurs a switching cost whenever their decision changes in consecutive time steps, i.e., when they increase or decrease their purchasing amount. We introduce competitive (robust) threshold-based algorithms for both the minimization and maximization variants of this problem, and show they are optimal among deterministic online algorithms. We then propose learning-augmented algorithms that take advantage of untrusted black-box advice (such as predictions from a machine learning model) to achieve significantly better average-case performance without sacrificing worst-case competitive guarantees. Finally, we empirically evaluate our proposed algorithms using a carbon-aware EV charging case study, showing that our algorithms substantially improve on baseline methods for this problem.

==> Z-relwork.tex <==
\adaml{we might not need a separate related work section since there is a lot of review of existing results throughout the paper?}

\note{rough scaffold here.  will enlist help from other folks}

\note{probably need:}

\note{paragraph(s) on related empirical work, including carbon aware scheduling, carbon intensity predictions, etc}

\note{paragraph(s) on MTS / SOCO type problems, including learn-aug stuff}

\note{paragraph(s) on online search type problems, including learn-aug stuff}

\note{a paragraph about pause and resume}

\note{a paragraph about advice complexity lit}


\adaml{transplanted from Section 2... needs some expansion}
Here we mention a few existing results which are most directly related to the problem setting of \PrOb.  
In the online search track of literature, prior work has shown learning-augmented algorithms for one-way trading~\cite{SunLee:21} and $k$-search~\cite{Lee:22}.  Both of these works design threshold-based algorithms which robustly incorporate advice in the form of a prediction about the ``best price'' which will be encountered throughout the input sequence, achieving the optimal trade-off between consistency and robustness.
From the online optimization perspective, learning-augmented approaches have been studied for convex function chasing and smoothed online convex optimization (\texttt{CFC/SOCO})~\cite{Christianson:22}, as well as metrical task systems (\texttt{MTS})~\cite{Antoniadis:20MTS, Christianson:23MTS}.  These works generally consider directly incorporating machine-learned predictions of the actual decision at each time step. 


==> temp-rate.tex <==






